Analogy Mining for Specific Design Needs

Finding analogical inspirations in distant domains is a powerful way of solving problems. However, as the number of inspirations that could be matched and the dimensions on which that matching could occur grow, it becomes challenging for designers to find inspirations relevant to their needs. Furthermore, designers are often interested in exploring specific aspects of a product-- for example, one designer might be interested in improving the brewing capability of an outdoor coffee maker, while another might wish to optimize for portability. In this paper we introduce a novel system for targeting analogical search for specific needs. Specifically, we contribute a novel analogical search engine for expressing and abstracting specific design needs that returns more distant yet relevant inspirations than alternate approaches.

==> deadKittens.tex <==
% \subsection{Design-By-Analogy}
% \jnote{Goals: 1) give some background on how analogy is useful in design, 2) nod to some other design-by-analogy methods, both "low-tech" stuff like TRIZ, Synectics, and WordTrees, and more advanced stuff like Kate Fu's bayesian structure learning stuff 3) set up our "redesign this product" scenario}
% \nnote{Hila maybe you could help here with analogy/design/product stuff you think is relevant?}

% Design-by-analogy is a big research topic. Much evidence that expert designers use analogies. Also, finding analogies from distant domains can give you more novel ideas, but sometimes at the cost of idea quality if the analogy is ``too far''.

% Lots of work trying to figure out how to create a \textit{systematic} process for drawing inspiration through analogy (often across domains).
% Many methods: TRIZ \cite{altshuller1984creativity}, Gordon's Synectics \cite{gordon_synectics:_1961}, Biologically inspired design, WordTree method \cite{linsey_design_2012} has people use the WordNet ontology to systematically ``walk up'' levels of abstraction for describing the core desired functionality. Pretty much a manual process. The goal is to get to a different level of abstraction for describing the problem so that we can think of other things that might be relevant from different domains.

%By abstraction, we mean generalizing a concept beyond its surface features while maintaining its core relational structure (cite). In the above, seeing the analogy between the steering of wings and the twisting of a cardboard box requires generalizing beyond the surface details of color or material to the similarity of the shearing forces when both wings and boxes are twisted.  Many real world solutions similarly require multiple different problem framings that would benefit from focusing and abstraction; for example, a coffee maker taken camping may benefit from distant inspirations that make it more lightweight, resistant to weather, a better grinder, or allow the camper to know when to pull it off the fire.

%Search engines that could support focused and abstracted analogical search for specific design needs could significantly increase the rate of innovation and problem solving today. The rise of knowledge databases and repositories on the Internet (e.g., the US Patent Database, Google Scholar, Amazon products, etc.) provides a virtual treasure trove of ideas that could inspire solutions across a variety of domains. 



% \subsection{\textcolor{red}{BEGIN ALT MOTIVATION FOCUSING ON THE PROBLEM OF HOW TO CONTROL ABSTRACTION (with properties) - BRANCH OFF AFTER DAFNA'S COMMENT ABOVE}}
% \subsection{\textcolor{red}{Challenges for Focus and Targeted Abstraction}}
% \textcolor{red}{Given a specific framing, it is not hard for search engines to find near analogies for that framing: for example, given the query ``lightweight approach for angling wings in opposite directions to steer the plane'', many state-of-the-art search engines could feasibly return many inspirations related to how steering mechanisms in planes. However, in many situations, designers benefit greatly by having inspirations from a diversity of domains, including those that are different from the problem domain (e.g., as in the The task of finding distant yet also relevant inspirations for the focused query, however, is significantly more challenging.}
% % 
% \textcolor{red}{In order to go beyond the domain of the problem, it is crucial to be able to effectively accomplish \textbf{abstraction}, by which we mean generalizing a concept beyond its surface features while maintaining its core relational structure \cite{}. One approach would be to ignore the entities entirely, and match only on the relations. For example, in the steering wings case, one might try to find matches related to the relations of \textit{angling} and \textit{steering}, and abstract away from (e.g., ignore) descriptions of the entities in the relations, like the \textit{wings} and \textit{plane}. Another approach might be to simply replace the core terms with their hypernyms, such as matching other things that are about \textit{controlling} some object (abstracting away from the physicality of steering/angling). These approaches to abstraction might enable a search engine to find many inspirations outside of the domain of planes; however, many of these inspirations are unlikely to be useful, e.g., \textit{steering} wheels in cars (which cannot suggest useful mechanisms for manipulating the angle of wings during flight), or actuarial methods for \textit{controlling} risk during insurance pricing. Without effective ways to abstract the core problem in a targeted manner (i.e., preserving all of the core relational structure), search engines face an unfavorable relevance/distance tradeoff: they can choose to return relevant matches for the specific information need for the designer (but remain restricted to ideas from the same domain, many of which the designer is likely already familiar with), \textit{or} attempt to abstract away from the details of the query and find distant matches, but end up forcing the designer to sift through many irrelevant search results.}
% %
% \textcolor{red}{Drawing on cognitive theories of analogy, we hypothesize that in order to find inspirations that are both domain distant and relevant, it is crucial to enable designers to express the key \textit{properties} of the relations and entities in the core relational structure. For example, in order to find inspirations that can suggest useful mechanisms for angling the wings (e.g., twisting of a cardboard box), need to express to the search engine that they don't care about the color and size of wings, but they \textit{do} care the fact that the wings are \textit{flat, physical objects}, or even that they are composed of materials that respond to \textit{shear forces} in a similar way to cardboard. \jnote{playing with the ``it's hard because how should we express this targeted abstraction to a machine?'' angle}.}

% \subsection{\textcolor{red}{END ALT MOTIVATION BRANCH}}

%\jnote{@Karni, moved this from the considerations section to be considered in context, but can't really make sense of it? Sounds to me like we're describing a hack here, as opposed to an interesting design choice we made through iteration (e.g., how we chose levels of abstraction to display during the abstraction step above). If we can't make this clearer, I suggest we drop this bit.}
%\knote{will try to make it clearer in the text. The design choice was not to make a special effort for this case as this is rare. I agree we should consider dropping as it really more like a footnote. The shortest rephrasing I can think of is:
%When abstracting the corpus, we assume a single sense per word since words usually have a predominant sense \cite{} .  The few exceptions such as ``bank'' as a a place by a river, or a financial institution  do not warrant special design effort. Moreover we expect that in such cases the surrounding words would reflect the context and make the overall effect negligible.}

%When abstracting the corpus, we faced the challenge of how to deal with ambiguities with respect to word sense (e.g., does the term ``bank'' refer to a place by a river, or a financial institution?). when selecting terms to replace with the designer's selected properties from the focus-abstracted query, we assume a single sense per term \jnote{within the same document?} , i.e., we assume that any other instance of that  term and any other term with those properties appear in the sense relevant to those properties. For example when abstracting soap to toiletry substance we assume that other instances of soap appear in the same sense and not, for example, in the sense of soap opera. This is reasonable as words usually have a predominant sense. \cite{}. The few exceptions such as "bank" mentioned above do not warrant special design effort as We expect that in such cases the surrounding words would reflect the context and make the overall effect negligible. 

%are two components to the analogy engine: a) a Representation Builder that takes the output of Step 3 as input and builds computational representations of the query and documents in the corpus that reflect the desired focus and abstraction, and b) a Matcher that uses those representations to find analogies for the query.
%Once the designer completes the focus and abstraction steps we invokes the analogy search engine for finding analogies for the particular need.

%Figure \ref{fig:ex-abstracting-corpus}. This component takes the output of Step 3 as input. This consists of a list of which sentences were selected as indicating the desired focus; for each sentence, the words (OR their chosen abstracted properties) in those sentences that are actually important (i.e., dropping words that were marked as IGNORE). The desired output is a set of vector representations of the query and all documents in the corpus, which the Matcher component can use to find analogies for the query.

%There are a number of possible methods for converting textual representations into vector representations that are suitable for similarity matching. For example \jnote{note a few}. Hope et al \cite{hope2017accelerating} introduced a method for creating specialized vector representations that are able to capture the overall \textit{purpose} of a given product, and showed that these vector representations are better for finding analogies compared to general vector representations like TF-IDF-aggregated GloVe vectors. \knote {I looked at this new description just briefly. I think there is a confusion here, as we use the  purpose function that was learnt, i.e., do not calculate it directly. Will look at it again in a couple of hours to make sure I understood your text correctly} Therefore, we use their method to convert the output of Step 3 into vector representations of the query and corpus that reflect the abstracted focus purpose chosen by the designer. This method takes a bag of words as input, and uses \jnote{self-contained concise description of how it works} to create a vector representation that captures the ``purpose'' of the query. The intuition is that this method gives more weight to ``purpose-like'' terms like 'need' and 'safe', and 'lightweight'. \jnote{note that this is somewhat specific to Quirky, but ok since it's in the same corpus?}

%Turning the query into a purpose vector representation is straightforward. The input consists of the entirety of the output of Step 3.\jnote{Karni, please make sure this is correct!} Representing the corpus to reflect the intended focus and abstraction is less straightforward. The goal is to make it possible for products that share similar purposes to the focus query to be matched as closer in the purpose vector space. \jnote{Maybe note a couple of more and less aggressive options?}. To accomplish this, we use the chosen abstractions from Step 3 to abstract all documents in the corpus.
%The engine first abstracts the entire Quirky corpus according to the input of Step 3. %It abstracts products or terms that share the properties deemed important by the designer to those properties.  
%\dnote{closing sentence about why we're doing this -- to make these other products closer}
